Data Assimilation and Sensitivity of the Black Sea Model to Parameters

An adjoint based technique is applied to a Shallow Water Model in order to estimate influence of the model's parameters on the solution. Among parameters the bottom topography, initial conditions, boundary conditions on rigid boundaries, viscosity coefficients and the amplitude of the wind stress tension are considered. Their influence is analyzed from different points of view. Two configurations have been analyzed: an academic case of the model in a square box and a more realistic case simulating Black Sea currents. It is shown in both experiments that the boundary conditions near a rigid boundary influence the most the solution. This fact points out the necessity to identify optimal boundary approximation during a model development.

==> 1d-grid-short.tex <==
 
\begin{figure}[h]
\setlength{\unitlength}{0.7mm}
\newcount\indi
\newcount\num
\tiny
\begin{picture}(80,20)
\Thicklines
\put(5,10){\line(1,0){80}}
\put(5,8){\line(0,1){4}}

\thicklines
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%U velocity (integer points)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\multiput(5,9)(15,0){4}{\line(0,1){2}}
\indi=-1
\multiput(2,6)(15,0){4}{ 
\global\advance\indi by 1 $u_{\the\indi}$ }


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%h height
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multiput(12,9)(15,0){3}{\line(1,1){2}}
\multiput(14,9)(15,0){3}{\line(-1,1){2}}
\indi=-1
\multiput(6,15)(15,0){3}{ 
\global\advance\indi by 1 \num=\indi \multiply\num by 2 \global\advance\num by 1 $\left.\der{u}{x}\right|_{\the\num/2}$ }

 \put(12,9){\line(1,1){2}}
\put(14,9){\line(-1,1){2}}
\end{picture} 
\end{figure}


